Seeing double through dependent optics

Tambara modules are strong profunctors between monoidal categories. They've been defined by Tambara in the context of representation theory, but quickly found their way in applications when it was understood Tambara modules provide a useful encoding of modular data accessors known as mixed optics. To suit the needs of these applications, Tambara theory has been extended to profunctors between categories receiving an action of a monoidal category. Motivated by the generalization of optics to dependently-typed contexts, we sketch a further extension of the theory of Tambara modules in the setting of actions of double categories (thus doubly indexed categories), by defining them as horizontal natural transformations. The theorems and constructions in Pastro-Street theory relevant to profunctor representation theorem for mixed optics are reobtained in this context. This reproduces the definition of dependent optics recently put forward by Vertechi and Milewski, and hinted at by previous work of the author and his collaborators.

==> src/dependent-lenses-and-charts.tex <==
\subsubsection{Deconstructing lenses and charts}
\matteo{shouldn't the domain of $p^\sharp$ be $q_*(z \times_x a)$?}
What's the 2-opfibration associated to $L$? One gets a category $\Para_L(\cat C)$ whose objects are pairs $(x, a \to x)$ of an object and an arrow over it in $\cat C$, and maps $(x, u: a \to x) \to (y, v : b \to y)$ are given by a span $x \nfrom{q} z \nto{p} y$ and a map $p^\sharp : z \times_x a \to b$ completing the following diagram:
% https://q.uiver.app/?q=WzAsNixbMCwwLCJiIl0sWzAsMSwieSJdLFsyLDAsImEiXSxbMiwxLCJ4Il0sWzEsMSwieiJdLFsxLDAsInogXFx0aW1lc194IGEiXSxbMCwxXSxbMiwzXSxbNCwzLCJwIiwyXSxbNCwxLCJxIl0sWzUsNF0sWzUsMl0sWzUsMCwicF5cXHNoYXJwIiwyXSxbNSwzLCIiLDIseyJzdHlsZSI6eyJuYW1lIjoiY29ybmVyIn19XV0=
\begin{equation}
\begin{tikzcd}
	b & {z \times_x a} & a \\
	y & z & x
	\arrow[from=1-1, to=2-1]
	\arrow[from=1-3, to=2-3]
	\arrow["p"', from=2-2, to=2-3]
	\arrow["q", from=2-2, to=2-1]
	\arrow[from=1-2, to=2-2]
	\arrow[from=1-2, to=1-3]
	\arrow["{p^\sharp}"', from=1-2, to=1-1]
	\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-2, to=2-3]
\end{tikzcd}
\end{equation}
The knowledgeable reader will recognize dependent lenses, but the careful reader will realize these morphisms are strictly more general than dependent lenses, since those are limited to $q = 1_y$.
That is, dependent lenses arise for specific choices of the span $x \nfrom{q} z \nto{p} y$, namely those of the form $x \equalto y \nto{p} y$.
We mention in passing that one can recognize in~\eqref{diag:action-of-category}, describing the action of a category, as a diagram of this form.

There is, after all, an embedding of $\cat C$ in $\Span(\cat C)$:
% https://q.uiver.app/?q=WzAsNyxbMCwzLCJ5Il0sWzAsMSwieCJdLFsyLDAsIlxcU3BhbihcXGNhdCBDKSJdLFswLDAsIlxcY2F0IEMiXSxbMiwxLCJ4Il0sWzIsMywieSJdLFszLDIsIngiXSxbMywyLCJcXGlvdGFeXFxlbGwiXSxbMSwwLCJwIiwyXSxbNiw1XSxbNCw2LCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs4LDYsIiIsMix7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0Ijo2MH0sImxldmVsIjoxLCJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV1d
\begin{equation}
\begin{tikzcd}[sep=4ex]
	{\cat C} &[3ex]&[-1ex] {\Span(\cat C)} &[-5ex] \\[-3ex]
	x && x \\[-2ex]
	&&& x \\[-2ex]
	y && y
	\arrow["{\iota^\ell}", from=1-1, to=1-3]
	\arrow[""{name=0, anchor=center, inner sep=0}, "p"', from=2-1, to=4-1]
	\arrow[from=3-4, to=4-3]
	\arrow[Rightarrow, no head, from=2-3, to=3-4]
	\arrow[shorten <=24pt, shorten >=40pt, maps to, from=0, to=3-4]
\end{tikzcd}
\end{equation}
It's now easy to recover dependent lenses, by taking the pullback of $L$ along $\iota^\ell$:
% https://q.uiver.app/?q=WzAsNCxbMSwwLCJcXGludCBMIl0sWzEsMSwiXFxTcGFuKFxcY2F0IEMpIl0sWzAsMSwiXFxjYXQgQyJdLFswLDAsIlxcRExlbnMoXFxjYXQgQykiXSxbMCwxLCJcXHBpIl0sWzIsMSwiXFxpb3RhXlxcZWxsIiwyXSxbMywyXSxbMywwXSxbMywxLCIiLDEseyJzdHlsZSI6eyJuYW1lIjoiY29ybmVyIn19XV0=
\begin{equation}
\begin{tikzcd}
	{\DLens(\cat C)} & {\int L} \\
	{\cat C} & {\Span(\cat C)}
	\arrow["\pi", from=1-2, to=2-2]
	\arrow["{\iota^\ell}"', from=2-1, to=2-2]
	\arrow[from=1-1, to=2-1]
	\arrow[from=1-1, to=1-2]
	\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-1, to=2-2]
\end{tikzcd}
\end{equation}
By the way, let us mention that there is also an embedding of $\cat C^\op$ in $\Span(\cat C)$, the \emph{right emebedding} $\iota^r$, given by sending a morphism $x \nto{q} y$ to the span $y \nfrom{q} x \equalto x$.
If we instead pullback along this functor, one gets a category analogous to $\int L$ whose morphisms are now restricted to diagrams of the form:
% https://q.uiver.app/?q=WzAsNixbMCwwLCJiIl0sWzAsMSwieSJdLFsyLDAsImEiXSxbMiwxLCJ4Il0sWzEsMSwieCJdLFsxLDAsImEiXSxbMCwxXSxbMiwzXSxbNCwzLCIiLDIseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDEsInEiXSxbNSw0XSxbNSwyLCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1LDAsInFeXFxmbGF0IiwyXSxbNSwzLCIiLDIseyJzdHlsZSI6eyJuYW1lIjoiY29ybmVyIn19XV0=
\begin{equation}
\begin{tikzcd}
	b & a & a \\
	y & x & x
	\arrow[from=1-1, to=2-1]
	\arrow[from=1-3, to=2-3]
	\arrow[Rightarrow, no head, from=2-2, to=2-3]
	\arrow["q", from=2-2, to=2-1]
	\arrow[from=1-2, to=2-2]
	\arrow[Rightarrow, no head, from=1-2, to=1-3]
	\arrow["{q^\flat}"', from=1-2, to=1-1]
	\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-2, to=2-3]
\end{tikzcd}
\end{equation}
These are known as `commuting squares' or more fancily as `dependent charts', since they are in one-to-one correspondence with diagrams of the form:
% https://q.uiver.app/?q=WzAsNixbMCwwLCJhIl0sWzAsMSwieCJdLFsyLDAsImIiXSxbMiwxLCJ5Il0sWzEsMSwieiJdLFsxLDAsInogXFx0aW1lc194IGIiXSxbMCwxXSxbMiwzXSxbNCwzLCJwIiwyXSxbNCwxLCIiLDAseyJsZXZlbCI6Miwic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs1LDRdLFs1LDJdLFswLDUsInBeXFxzaGFycCJdLFs1LDMsIiIsMix7InN0eWxlIjp7Im5hbWUiOiJjb3JuZXIifX1dXQ==
\begin{equation}
\begin{tikzcd}
	a & {z \times_x b} & b \\
	x & z & y
	\arrow[from=1-1, to=2-1]
	\arrow[from=1-3, to=2-3]
	\arrow["p"', from=2-2, to=2-3]
	\arrow[Rightarrow, no head, from=2-2, to=2-1]
	\arrow[from=1-2, to=2-2]
	\arrow[from=1-2, to=1-3]
	\arrow["{p^\sharp}", from=1-1, to=1-2]
	\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-2, to=2-3]
\end{tikzcd}
\end{equation}
which are the dependently-typed generalisation of charts \cite{myers2021book}.
Hence we obtain $\cat C^\op \times_{\Span(\cat C)} \int L \iso \DChart(\cat C)^\op$.

